On Leveraging Encoder-only Pre-trained Language Models for Effective Keyphrase Generation

This study addresses the application of encoder-only Pre-trained Language Models (PLMs) in keyphrase generation (KPG) amidst the broader availability of domain-tailored encoder-only models compared to encoder-decoder models. We investigate three core inquiries: (1) the efficacy of encoder-only PLMs in KPG, (2) optimal architectural decisions for employing encoder-only PLMs in KPG, and (3) a performance comparison between in-domain encoder-only and encoder-decoder PLMs across varied resource settings. Our findings, derived from extensive experimentation in two domains reveal that with encoder-only PLMs, although KPE with Conditional Random Fields slightly excels in identifying present keyphrases, the KPG formulation renders a broader spectrum of keyphrase predictions. Additionally, prefix-LM fine-tuning of encoder-only PLMs emerges as a strong and data-efficient strategy for KPG, outperforming general-domain seq2seq PLMs. We also identify a favorable parameter allocation towards model depth rather than width when employing encoder-decoder architectures initialized with encoder-only PLMs. The study sheds light on the potential of utilizing encoder-only PLMs for advancing KPG systems and provides a groundwork for future KPG methods. Our code and pre-trained checkpoints are released at https://github.com/uclanlp/DeepKPG.

==> tables/bert2bert_enc_feature_quality.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[!t]
    \small
    % \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l | c | c c | c c  }
    \hline
    \multirow{2}{*}{Model Size} & \multirow{2}{*}{|M|} & \multicolumn{2}{c|}{\textbf{freeze+CRF}} & \multicolumn{2}{c}{\textbf{unfreeze}} \\
    & & F1@5 & F1@M & F1@5 & F1@M \\
    \hline
    2 layers & 39M & 19.2 & 30.5 & 31.5 & 45.2 \\
    4 layers & 53M & 26.5 & 38.1 & 32.6 & 46.7 \\
    6 layers & 67M & \textbf{27.4} & \textbf{39.1} & 33.2 & 47.8 \\
    8 layers & 81M & 26.8 & 38.7 & \textbf{34.4} & \textbf{48.5} \\
    10 layers & 95M & 26.9 & 38.3 & 33.0 & 47.9 \\
    \hline
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{
    The feature quality of the encoders via sequence labeling results on the KPTimes test set. The models are the encoders taken from BERT2BERT models trained on keyphrase generation and further trained on keyphrase extraction on KPTimes. "freeze" means freezing the underlying encoder model while "unfreeze" means fine-tuning the entire model. For the unfreeze version we found using CRF unnecessary.
    }
    \label{tab:feature_quality_b2b_enc}
    % \vspace{-2mm}
\end{table}

==> tables/keyphrase_generation_main_results.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[]
    \small
    \centering
    \resizebox{\linewidth}{!} {%
    \begin{tabular}{l | c | c c | c c  }
    \hline
    \multirow{2}{*}{Method} &
    \multirow{2}{*}{|M|} & \multicolumn{2}{c|}{\textbf{KP20k}} & \multicolumn{2}{c}{\textbf{KPTimes}} \\
    & & F1@5 & F1@M & F1@5 & F1@M \\
    \hline
    \multicolumn{4}{l}{\textbf{Present keyphrase generation}} \\ 
    \hline
    CatSeq & 21M & 29.1 & 36.7 & 29.5 & 45.3 \\
    ExHiRD-h & 22M & 31.1 & 37.4 & 32.1 & 45.2 \\
    Transformer & 98M & 33.3 & 37.6 & 30.2 & 45.3 \\
    SetTrans & 98M & \textbf{35.6} & 39.1 & 35.6 & 46.3 \\
    \hdashline
    \multirow{2}{*}{BART} & 140M & 32.2 & 38.8 & 35.9 & 49.9 \\
     & 406M & 33.2 & 39.2 & \textbf{37.3} & \textbf{51.0} \\
    \hdashline
    \multirow{2}{*}{T5} & 223M & 33.6 & 38.8 & 34.6 & 49.2 \\
     & 770M & 34.3 & \textbf{39.3} & 36.6 & 50.8 \\
    \hline
    \multicolumn{4}{l}{\textbf{Absent keyphrase generation}} \\ 
    \hline
    CatSeq & 21M & 1.5 & 3.2 & 15.7 & 22.7 \\
    ExHiRD-h & 22M & 1.6 & 2.5 & 13.4 & 16.5 \\
    Transformer & 98M & 2.2 & 4.6 & 17.1 & 23.1 \\
    SetTrans & 98M & \textbf{3.5} & \textbf{5.8} & \textbf{19.8} & 21.9 \\
    \hdashline
    \multirow{2}{*}{BART} & 140M & 2.2 & 4.2 & 17.1 & \textbf{24.9} \\
     & 406M & 2.7 & 4.7 & 17.6 & 24.4 \\
    \hdashline
    \multirow{2}{*}{T5} & 223M & 1.7 & 3.4 & 15.3 & 24.2 \\
     & 770M & 1.7 & 3.5 & 15.7 & 24.1 \\ 
    \hline
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{
    Keyphrase generation performance of task-specific neural methods and fine-tuning seq2seq PLMs. The best results are boldfaced. Large-sized BART and T5 approach the performance of SetTrans on KP20k and obtain the state-of-the-art F1@M on KPTimes.
    }
    \label{tab:main-kpg-results}
    % \vspace{-2mm}
\end{table}



==> tables/scibart_vs_keybart.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[!t]
    \small
    \centering
    \begin{tabular}{l | c | c c | c c  }
    \hline
    \multirow{2}{*}{Model} & \multirow{2}{*}{|M|} & \multicolumn{2}{c|}{\textbf{Present KPs}} & \multicolumn{2}{c}{\textbf{Absent KPs}} \\
    & & F1@5 & F1@M & F1@5 & F1@M \\
    \hline
    \multicolumn{6}{l}{\textbf{Zero-shot transfer from OAGKX}}\\
    \hline
    KeyBART & 406M & 20.4 & 22.8 & 1.7 & 0.9 \\
    \hdashline
    \multirow{2}{*}{SciBART$^\dagger$} & 124M & 26.6 & 31.2 & 1.5 & 2.6 \\
    & 386M & 23.5 & 28.5 & 1.3 & 2.3 \\
    \hline
    \multicolumn{6}{l}{\textbf{Fine-tuned on KP20k}}\\
    \hline
    KeyBART+ft & 406M & 32.5 & 39.8 & 2.6 & 4.7 \\ 
    \hdashline
    \multirow{2}{*}{SciBART+ft} & 124M & 34.1 & 39.6 & 2.9 & 5.2 \\
    & 386M & 34.7 & 41.5 & 3.1 & 5.7 \\
    \hdashline
    \multirow{2}{*}{SciBART$^\dagger$+ft} & 124M & 35.3 & 41.5 & 2.8 & 5.2 \\
    & 386M & \textbf{36.2} & \textbf{43.2} & \textbf{3.2} & \textbf{6.2} \\    
    \hline
    \end{tabular}
    \vspace{-2mm}
    \caption{
    Comparison between SciBART and KeyBART in zero-shot and fine-tuned settings. Both KeyBART and SciBART$^\dagger$ are first trained on OAGKX to learn to generate keyphrases. $^\dagger$ denotes the SciBART fine-tuned on OAGKX. "+ft" means fine-tuned on KP20k. 
    }
    \label{tab:scibart_vs_keybart}
    % \vspace{-2mm}
\end{table}

